Algebraically Explainable Controllers: Decision Trees and Support Vector Machines Join Forces

Recently, decision trees (DT) have been used as an explainable representation of controllers (a.k.a. strategies, policies, schedulers). Although they are often very efficient and produce small and understandable controllers for discrete systems, complex continuous dynamics still pose a challenge. In particular, when the relationships between variables take more complex forms, such as polynomials, they cannot be obtained using the available DT learning procedures. In contrast, support vector machines provide a more powerful representation, capable of discovering many such relationships, but not in an explainable form. Therefore, we suggest to combine the two frameworks in order to obtain an understandable representation over richer, domain-relevant algebraic predicates. We demonstrate and evaluate the proposed method experimentally on established benchmarks.

==> chapters/08_future_work.tex <==
% !TeX root = ../paper.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.

\section{Future Work} \label{chapter:future_work}
The tool \dtcontrol achieves great performance generating compact decision trees, especially when using the determination heuristics proposed in \cite{dtControl,dtcontrol2}. In this work, we showed that more expressive quadratic polynomials can especially help generate succinct trees for most-permissive controllers. An important part that can still be improved upon, however, is the explainability. Of course, succinct decision trees are already easier to understand by nature, but more complex predicates again reduce explainability. Ideally, we would want to have a justification explaining the coefficients of the complex predicate. Also, synthesizing other types of functions and improving the current curve fitting are interesting directions for future work.

\paragraph{Predicate Generation From Domain Knowledge}
We have seen that predicate generation from general domain knowledge without an effective heuristic is infeasible. If existent, such a heuristic would probably have to use a completely different approach, as the impurity approach taken in this thesis does not seem to be a promising choice. With regards to the problem of uniqueness we discovered in \autoref{sec:identified_problems}, a key component for a heuristic might be the model checker or at least the dynamics equations of the system. With that, simulations could be used to judge if a predicate describes a relevant behavior of the system. 

A different approach would be to use the polynomials we found in this work. Specifically, if we exactly know the coefficients where we want to arrive, it might be easier to find a derivation for that with some kind of meet-in-the-middle technique.

\paragraph{Feature Importance}
As we have described in \autoref{sec:featureImportance}, the proposed feature importance is far from perfect. The current implementation depends on the order of features. Future work could analyze this dependence and propose countermeasures. In the bigger picture, the feature importance could be lifted from a binary \enquote{relevant}/\enquote{irrelevant} classification to a continuous spectrum that could be used in the decision tree construction. 


\paragraph{Decision Tree Balance}
We proposed the min-label entropy impurity measure that focuses on separating one label first. As a result, we encourage the formation of unbalanced, line-like decision trees (see \autoref{sec:eval_mle}). However, more balanced decision trees might be easier to understand by a human. Additionally, we might reduce the individual predicate complexity (number of terms in the polynomial) if we use more general splits first. For that, we would need to develop an impurity measure that prefers split A from \autoref{fig:entropy_split_future} over split B, just like the standard entropy does, but still keeps the advantages of the min-label entropy and finds trees of minimum size.

\ifdefined\pics
\begin{figure}[ht]
  \centering
  \input{figures/entropy_split_future.tex}
  \caption{Two different splits with their respective min-label entropy (MLE) and standard entropy values. Split A leads to a more balanced tree and has a better entropy value but split B is preferred by the min-label entropy as one label is completely separated.}
  \label{fig:entropy_split_future}
\end{figure}
\fi

\paragraph{More Expressive Predicates}
In this work, we restricted ourselves to quadratic polynomials as predicates generated by the support vector machines. To mitigate the problems we discussed in \autoref{sec:problemsWithHigherDimensions}, techniques such as principal component analysis could be used to significantly reduce the dimensionality. This would allow us to use higher degree polynomials, maybe even other types of functions.

\paragraph{Analysis of Other Case Studies}
The \cruise model has been extensively discussed in other work \cite{sos, weinhuber, dtcontrol2} as well as this thesis and we have found adequate solutions. However, for case studies such as \t{helicopter} \cite{Jagtap2020} and \t{aircraft} \cite{Rungger2015} the decision tree representation is still larger than the BDD representation (see Appendix \ref{chp:all_results}). A better understanding of the model could lead to new realizations. Maybe other types of functions as predicates are needed or our impurity measures do not work sufficiently well for those cases.

\paragraph{Improved Curve Fitting}
In \autoref{sec:problem_with_curve_fitting} we show the difference between the current curve-fitting implementation and our new approach. In principle, the current approach uses regression analysis to find a function that fits the data with least-square-fitting. Our approach, however, tries to find a function separating the data instead of fitting it. As we have seen great success with our approach, we might be able to transfer some insight to the general curve fitting that is used to determine unspecified constants in user-entered expressions.


==> chapters/99_example.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.

\chapter{Introduction}\label{chapter:introduction}

\section{Section}
Citation test~\parencite{latex}.

\subsection{Subsection}

See~\autoref{tab:sample}, \autoref{fig:sample-drawing}, \autoref{fig:sample-plot}, \autoref{fig:sample-listing}.

\begin{table}[htpb]
  \caption[Example table]{An example for a simple table.}\label{tab:sample}
  \centering
  \begin{tabular}{l l l l}
    \toprule
      A & B & C & D \\
    \midrule
      1 & 2 & 1 & 2 \\
      2 & 3 & 2 & 3 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{figure}[htpb]
  \centering
  % This should probably go into a file in figures/
  \begin{tikzpicture}[node distance=3cm]
    \node (R0) {$R_1$};
    \node (R1) [right of=R0] {$R_2$};
    \node (R2) [below of=R1] {$R_4$};
    \node (R3) [below of=R0] {$R_3$};
    \node (R4) [right of=R1] {$R_5$};

    \path[every node]
      (R0) edge (R1)
      (R0) edge (R3)
      (R3) edge (R2)
      (R2) edge (R1)
      (R1) edge (R4);
  \end{tikzpicture}
  \caption[Example drawing]{An example for a simple drawing.}\label{fig:sample-drawing}
\end{figure}

\begin{figure}[htpb]
  \centering

  \pgfplotstableset{col sep=&, row sep=\\}
  % This should probably go into a file in data/
  \pgfplotstableread{
    a & b    \\
    1 & 1000 \\
    2 & 1500 \\
    3 & 1600 \\
  }\exampleA
  \pgfplotstableread{
    a & b    \\
    1 & 1200 \\
    2 & 800 \\
    3 & 1400 \\
  }\exampleB
  % This should probably go into a file in figures/
  \begin{tikzpicture}
    \begin{axis}[
        ymin=0,
        legend style={legend pos=south east},
        grid,
        thick,
        ylabel=Y,
        xlabel=X
      ]
      \addplot table[x=a, y=b]{\exampleA};
      \addlegendentry{Example A};
      \addplot table[x=a, y=b]{\exampleB};
      \addlegendentry{Example B};
    \end{axis}
  \end{tikzpicture}
  \caption[Example plot]{An example for a simple plot.}\label{fig:sample-plot}
\end{figure}

\begin{figure}[htpb]
  \centering
  \begin{tabular}{c}
  \begin{lstlisting}[language=SQL]
    SELECT * FROM tbl WHERE tbl.str = "str"
  \end{lstlisting}
  \end{tabular}
  \caption[Example listing]{An example for a source code listing.}\label{fig:sample-listing}
\end{figure}

